Transfer Learning for Non-Intrusive Load Monitoring

Non-intrusive load monitoring (NILM) is a technique to recover source appliances from only the recorded mains in a household. NILM is unidentifiable and thus a challenge problem because the inferred power value of an appliance given only the mains could not be unique. To mitigate the unidentifiable problem, various methods incorporating domain knowledge into NILM have been proposed and shown effective experimentally. Recently, among these methods, deep neural networks are shown performing best. Arguably, the recently proposed sequence-to-point (seq2point) learning is promising for NILM. However, the results were only carried out on the same data domain. It is not clear if the method could be generalised or transferred to different domains, e.g., the test data were drawn from a different country comparing to the training data. We address this issue in the paper, and two transfer learning schemes are proposed, i.e., appliance transfer learning (ATL) and cross-domain transfer learning (CTL). For ATL, our results show that the latent features learnt by a `complex' appliance, e.g., washing machine, can be transferred to a `simple' appliance, e.g., kettle. For CTL, our conclusion is that the seq2point learning is transferable. Precisely, when the training and test data are in a similar domain, seq2point learning can be directly applied to the test data without fine tuning; when the training and test data are in different domains, seq2point learning needs fine tuning before applying to the test data. Interestingly, we show that only the fully connected layers need fine tuning for transfer learning. Source code can be found at https://github.com/MingjunZhong/transferNILM.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> tables/results/refit-tl-comp.tex <==
\begin{table*}[htbp]
\caption{Appliance transfer learning for sequence-to-point learning. W.M. denotes Washing Machine.}
                \centering
                \scalebox{1}{
                \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
                %\hline
                % \multicolumn{7}{|>{\rowcolor{blue!10}}c|}{Appliance transfer learning results on REFIT (washing machine CNN)}
                %\rowcolor{blue!10}
                %\multicolumn{7}{|c|}{Appliance transfer learning results on REFIT (washing machine CNN)}    \\
                %\hline
                %Appliances         &  \multicolumn{6}{|c|}{Results}\\
                %\columncolor{green!50}
                \hline
                       & \multicolumn{4}{|>{}c|}
                        {AFHMM} & \multicolumn{4}{|>{}c|}
                        {Trained on REFIT}&  \multicolumn{4}{|>{}c|}{CNN trained on REFIT (using W.M.)}\\
                         
                        & \multicolumn{4}{|>{}c|}
                        {} &  \multicolumn{4}{|>{}c|}{Tested on REFIT}&  \multicolumn{4}{|>{}c|}{Tested on REFIT}\\
                \hline
                                     &\multicolumn{1}{|c|}{MAE}&\multicolumn{1}{|c|}{SAE}& \multicolumn{1}{|c|}{EpD [Wh]}&\multicolumn{1}{|c|}{NDE}&\multicolumn{1}{|c|}{MAE}&\multicolumn{1}{|c|}{SAE}& \multicolumn{1}{|c|}{EpD [Wh]}&\multicolumn{1}{|c|}{NDE}&\multicolumn{1}{|c|}{MAE} & \multicolumn{1}{|c|}{SAE}&\multicolumn{1}{|c|}{EpD [Wh]}&\multicolumn{1}{|c|}{NDE}\\
                \hline
                Kettle      &74.37 &2.41 &1203.52 &2.17    &6.830    &0.130   &153.92& 0.52  &12.690    &0.050   &96.04 &0.20 \\
                \hline
                Microwave   &12.25 &0.84 &276.90 &0.99   &12.660    &0.170   &95.78 &0.71   &13.380    &0.050   &107.730&0.70 \\
                \hline
                Fridge   &61.12 &0.99 &1305.55 &0.99       &20.020    &0.330   &216.85 & 0.43   &20.560    &0.440   &270.48 &0.45  \\
                \hline
                Dish w.   &163.79 &1.10 &3238.71 &5.12  &12.260   &0.260   &180.00 &0.44  &12.360   &0.610   &206.15 & 0.49\\
                \hline
                Washing m. &48.09 &0.80 &866.02 &1.47 &16.850    &2.610   &319.11 &0.54   &16.850    &2.610   &319.11 & 0.54\\
                \hline
                Overall   &71.92 &2.88  &1378.14 &2.15  & 13.724    & 0.702      & 193.13 &0.52 & 15.168    &0.752      &149.62 &0.47   \\
                mean $\pm$ std &50.38 &3.68 &997.24 &1.55  & 4.477    & 0.957      &74.32 &0.11  & 3.135    &0.955      &87.765 &0.18  \\
                \hline
                \end{tabular}
                }
                
                \label{tab:tabrestransF}
            \end{table*}

==> tikz_graphs/CNN_transfer.tex <==
        \begin{tikzpicture}
            \centering
            \node (one)[blockb]{CNN\\low level features};
            \node (two)[blockg,right of=one, xshift=4cm]{CNN\\high level features};
            \node (three)[block1,right of=two, xshift=4cm]{Fully\\connected layers};
            \draw[->] ($(one.north east)!0.5!(one.south east)$) -- node[below] {} ($(two.north west)!0.5!(two.south west)$);
            \draw[->] ($(two.north east)!0.5!(two.south east)$) -- node[below] {} ($(three.north west)!0.5!(three.south west)$);
        \end{tikzpicture}

==> tikz_graphs/neural_network.tex <==
\begin{figure}
    \centering
    %\scalebox{0.5}{
        \begin{tikzpicture}[
            plain/.style={
              draw=none,
              fill=none,
              },
            net/.style={
              matrix of nodes,
              nodes={
                draw,
                circle,
                inner sep=8pt
                },
              nodes in empty cells,
              column sep=0.2cm,
              row sep=-5pt
              },
            >=latex
            ]
            \matrix[net] (mat)
            {
            |[plain]| \parbox{1.3cm}{\centering Input\\layer} & |[plain]| \parbox{1.3cm}{\centering Hidden\\layer} & |[plain]| \parbox{1.3cm}{\centering Output\\layer} \\
            & |[plain]| \\
            |[plain]| & \\
            & |[plain]| \\
              |[plain]| & |[plain]| \\
            & & \\
              |[plain]| & |[plain]| \\
            & |[plain]| \\
              |[plain]| & \\
            & |[plain]| \\    };
            \foreach \ai [count=\mi ]in {2,4,...,10}
              \draw[<-] (mat-\ai-1) -- node[above] {Input \mi} +(-2cm,0);
            \foreach \ai in {2,4,...,10}
            {\foreach \aii in {3,6,9}
              \draw[->] (mat-\ai-1) -- (mat-\aii-2);
            }
            \foreach \ai in {3,6,9}
              \draw[->] (mat-\ai-2) -- (mat-6-3);
            \draw[->] (mat-6-3) -- node[above] {Ouput} +(2cm,0);
        \end{tikzpicture}
        %}
    \caption{Neural network example}
    \label{fig:neunetex}
\end{figure}

==> tikz_graphs/neuron.tex <==
\usetikzlibrary{matrix,chains,positioning,decorations.pathreplacing,arrows}   

    \begin{figure}
        \centering
            \begin{tikzpicture}[
            init/.style={
              draw,
              circle,
              inner sep=2pt,
              font=\Huge,
              join = by -latex
            },
            squa/.style={
              draw,
              inner sep=2pt,
              font=\Large,
              join = by -latex
            },
            start chain=2,node distance=8mm
            ]
            \node[on chain=2] 
              (x2) {$x_2$};
            \node[on chain=2,join=by -latex] 
              {$w_2$};
            \node[on chain=2,init] (sigma) 
              {$\displaystyle\Sigma$};
            \node[on chain=2,squa,label=above:{\parbox{2cm}{\centering Activate \\ function}}]   
              {$f$};
            \node[on chain=2,label=above:Output,join=by -latex] 
              {$y$};
            \begin{scope}[start chain=1]
            \node[on chain=1] at (0,1.5cm) 
              (x1) {$x_1$};
            \node[on chain=1,join=by -latex] 
              (w1) {$w_1$};
            \end{scope}
            \begin{scope}[start chain=3]
            \node[on chain=3] at (0,-1.5cm) 
              (x3) {$x_3$};
            \node[on chain=3,label=below:Weights,join=by -latex] 
              (w3) {$w_3$};
            \end{scope}
            \node[label=above:\parbox{2cm}{\centering Bias \\ $b$}] at (sigma|-w1) (b) {};
            \draw[-latex] (w1) -- (sigma);
            \draw[-latex] (w3) -- (sigma);
            \draw[-latex] (b) -- (sigma);
            \draw[decorate,decoration={brace,mirror}] (x1.north west) -- node[left=10pt] {Inputs} (x3.south west);
            \end{tikzpicture}
            
            
        \caption{Single neuron structure and mathematical representation}
        \label{fig:neuron}
    \end{figure}

==> tikz_graphs/nilm_types.tex <==
    \begin{tikzpicture}
          [
            ->,
            >=Stealth,
            shorten >=1pt,
            shorten <=1pt,
            thick,
            main node/.style={fill=white, draw, font=\sffamily\scriptsize\bfseries, blur shadow, align=center},
            hex/.style={main node, chamfered rectangle},
            ell/.style={main node, ellipse},
            blur shadow={shadow opacity=15},
            start chain=main going below,
          ]
          \node [on chain, ell] {Sample Frequency};
          {[start branch=a going {at=(main-1), shift=({35-(\tikzchaincount-1)*20}:3)}, every on chain/.append style={join={with main-1 by ->}}]
            \node [on chain, ell] {Low frequency};
            \node [on chain, ell] {High \\ frequency};
            }
          \node [on chain, ell] {Appliance feature \\ extraction};
          {[start branch=b going {at=(main-2), shift=({30-(\tikzchaincount-1)*20}:3)}, every on chain/.append style={join={with main-2 by ->}}]
            \node [on chain, ell] {Stady State};
            \node [on chain, ell] {Transient};
            \node [on chain, ell] {Hybrid};
             }
            %add , join=by - to \node[on chain, ell, join=by -] for link 
            \node [on chain, ell] {Inference and\\ learning};
           {[start branch=ep going {at=(main-3), shift=({0-(\tikzchaincount-1)*20}:3)}, every on chain/.append style={join={with main-3 by ->}}]
            \node [on chain, ell] {Supervised};
            \node [on chain, ell] {Unsupervised};
             }
        \end{tikzpicture}
